CvxNet: Learnable Convex Decomposition

Any solid object can be decomposed into a collection of convex polytopes (in short, convexes). When a small number of convexes are used, such a decomposition can be thought of as a piece-wise approximation of the geometry. This decomposition is fundamental in computer graphics, where it provides one of the most common ways to approximate geometry, for example, in real-time physics simulation. A convex object also has the property of being simultaneously an explicit and implicit representation: one can interpret it explicitly as a mesh derived by computing the vertices of a convex hull, or implicitly as the collection of half-space constraints or support functions. Their implicit representation makes them particularly well suited for neural network training, as they abstract away from the topology of the geometry they need to represent. However, at testing time, convexes can also generate explicit representations -- polygonal meshes -- which can then be used in any downstream application. We introduce a network architecture to represent a low dimensional family of convexes. This family is automatically derived via an auto-encoding process. We investigate the applications of this architecture including automatic convex decomposition, image to 3D reconstruction, and part-based shape retrieval.

==> fig/onecol.tex <==
\begin{figure}
\centering
\begin{overpic} 
[width=\linewidth]
% [width=\linewidth,grid,tics=10]
{fig/onecol.pdf}
% \myfigurename{}
\end{overpic}
\caption{
% 
One column template
% 
}
\label{fig:onecol}
\end{figure}

==> fig/twincol.tex <==
\newcommand\subfigw{.49}
\begin{figure*}
% --------------
% --------------
% --------------
\begin{minipage}[t]{\subfigw\linewidth}
\begin{overpic} 
[width=\linewidth]
% [width=\linewidth,grid,tics=10]
{fig/onecol.pdf}
\myfigurenametwin{}
\end{overpic}
\caption{
% 
TwinColumn left caption.
% 
}
\label{fig:twincol-l}
\end{minipage}%
$\hfill$
\begin{minipage}[t]{\subfigw\linewidth}
\begin{overpic} 
[width=\linewidth]
% [width=\linewidth,grid,tics=10]
{fig/onecol.pdf}
\end{overpic}
\caption{
% 
TwinColumn right caption.
% 
}
\label{fig:twincol-r}
\end{minipage}
\end{figure*}

==> fig/twocol.tex <==
\begin{figure*}[ht]
\centering
\begin{overpic} 
[width=\linewidth]
% [width=\linewidth,grid,tics=10]
{fig/twocol.pdf}
% \myfigurename{}
\end{overpic}
\caption{
% 
Two column template
% 
}
\label{fig:twocol}
\end{figure*}


==> tab/shapenet-v2.tex <==
% \newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\begin{table*}
\begin{center}
\setlength\tabcolsep{3pt} % default value: 6pt
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc} 
\toprule
\multirow{2}{*}{Category} & \multicolumn{3}{c}{IoU}                    & \multicolumn{3}{c}{Chamfer-$L_1$ }                 & \multicolumn{3}{c}{F-Score}                \\
                          & OccNet         & SIF     & Ours            & OccNet          & SIF            & Ours   & OccNet& SIF   & Ours             \\ 
\midrule
airplane                  & \textbf{0.759} & 0.662   & 0.739           & \textbf{0.017}  & 0.044          & 0.025  & \textbf{86.5} & 71.40 & 84.68   \\
bench                     & \textbf{0.714} & 0.533   & 0.631           & \textbf{0.020}  & 0.082          & 0.043  & \textbf{86.1} & 58.35 & 77.68   \\
cabinet                   & \textbf{0.861} & 0.783   & 0.830           & \textbf{0.045}  & 0.110          & 0.048  & \textbf{85.3} & 59.26 & 76.09   \\
car                       & \textbf{0.831} & 0.772   & 0.826           & 0.064           & 0.108          & \textbf{0.031}  & 75.8 & 56.58 & \textbf{77.75}   \\
chair                     & \textbf{0.732} & 0.572   & 0.681           & \textbf{0.044}  & 0.154          & 0.115  & \textbf{75.2} & 42.37 & 65.39   \\
display                   & \textbf{0.814} & 0.693   & 0.762           & \textbf{0.035}  & 0.097          & 0.065  & \textbf{81.4} & 56.26 & 71.41   \\
lamp                      & \textbf{0.565} & 0.417   & 0.494           & \textbf{0.157}  & 0.342          & 0.352  & \textbf{61.6} & 35.01 & 51.37            \\
speaker                   & 0.691          & 0.742   & \textbf{0.784}  & \textbf{0.019}  & 0.199          & 0.112  & \textbf{84.0} & 47.39 & 60.24   \\
rifle                     & \textbf{0.869} & 0.604   & 0.684           & 0.031           & 0.042          & \textbf{0.023}  & \textbf{84.5} & 70.01 & 83.63   \\
sofa                      & 0.823          & 0.760   & \textbf{0.828}  & 0.107           & 0.080          & \textbf{0.036}  & 73.9 & 55.22 & \textbf{75.44}   \\
table                     & \textbf{0.756} & 0.572   & 0.660           & \textbf{0.038}  & 0.157          & 0.121  & \textbf{84.1} & 55.66 & 71.73   \\
phone                     & \textbf{0.911} & 0.831   & 0.869           & \textbf{0.013}  & 0.039          & 0.018  & \textbf{94.0} & 81.82 & 89.28   \\
vessel                    & \textbf{0.745} & 0.643   & 0.708           & \textbf{0.042}  & 0.078          & 0.052  & \textbf{75.6} & 54.15 & 70.77   \\ 
\midrule     
mean                      & \textbf{0.775}  & 0.660  & 0.731 & \textbf{0.049} & 0.118     & 0.080  & \textbf{80.6} & 59.02 & 73.49   \\
\bottomrule
\multicolumn{10}{c}{\textbf{\{Depth\}-to-3D}}


\end{tabular}
% 
\hspace{.1in}
% 
\begin{tabular}{l|ccccc|ccccc|cccc} 
\toprule
\multirow{2}{*}{Category} & \multicolumn{5}{c}{IoU}                                      & \multicolumn{5}{c}{Chamfer-$L_1$ }                                            & \multicolumn{4}{c}{F-Score}                                   \\
                          & P2M   & AtlasNet & OccNet          & SIF   & Ours            & P2M   & AtlasNet        & OccNet          & SIF             & Ours            & AtlasNet        & OccNet           & SIF   & Ours             \\ 
\midrule
airplane                  & 0.420 & -        & 0.571           & 0.530 & \textbf{0.598}   & 0.187 & 0.104           & 0.147            & 0.167 & \textbf{0.093}  & 67.24           & 62.87            & 52.81 & \textbf{68.16}   \\
bench                     & 0.323 & -        & \textbf{0.485}  & 0.333 & 0.461            & 0.201 & 0.138           & 0.155            & 0.261 & \textbf{0.133}  & 54.50           & \textbf{56.91}   & 37.31 & 54.64            \\
cabinet                   & 0.664 & -        & \textbf{0.733}  & 0.648 & 0.709            & 0.196 & 0.175           & 0.167            & 0.233 & \textbf{0.160 } & 46.43           & \textbf{61.79}   & 31.68 & 46.09            \\
car                       & 0.552 & -        & \textbf{0.737}  & 0.657 & 0.675            & 0.180 & 0.141           & 0.159            & 0.161 & \textbf{0.103}  & 51.51           & \textbf{56.91}   & 37.66 & 47.33            \\
chair                     & 0.396 & -        & \textbf{0.501}  & 0.389 & 0.491            & 0.265 & \textbf{0.209 } & 0.228            & 0.380 & 0.337           & 38.89           & \textbf{42.41}   & 26.90 & 38.49            \\
display                   & 0.490 & -        & 0.471           & 0.491 & \textbf{0.576}   & 0.239 & \textbf{0.198}  & 0.278            & 0.401 & 0.223           & \textbf{42.79}  & 38.96            & 27.22 & 40.69            \\
lamp                      & 0.323 & -        & \textbf{0.371}  & 0.260 & 0.311            & 0.308 & \textbf{0.305}  & 0.479            & 1.096 & 0.795           & 33.04           & \textbf{38.35}   & 20.59 & 31.41            \\
speaker                   & 0.599 & -        & \textbf{0.647}  & 0.577 & 0.620            & 0.285 & \textbf{0.245}  & 0.300            & 0.554 & 0.462           & 35.75           & \textbf{42.48}   & 22.42 & 29.45            \\
rifle                     & 0.402 & -        & 0.474           & 0.463 & \textbf{0.515 }  & 0.164 & 0.115           & 0.141            & 0.193 & \textbf{0.106}  & \textbf{64.22}  & 56.52            & 53.20 & 63.74            \\
sofa                      & 0.613 & -        & \textbf{0.680}  & 0.606 & 0.677            & 0.212 & 0.177           & 0.194            & 0.272 & \textbf{0.164}  & 43.46           & \textbf{48.62}   & 30.94 & 42.11            \\
table                     & 0.395 & -        & \textbf{0.506}  & 0.372 & 0.473            & 0.218 & 0.190           & \textbf{0.189 }  & 0.454 & 0.358           & 44.93           & \textbf{58.49}   & 30.78 & 48.10            \\
phone                     & 0.661 & -        & \textbf{0.720}  & 0.658 & 0.719            & 0.149 & 0.128           & 0.140            & 0.159 & \textbf{0.083}  & 58.85           & \textbf{66.09}   & 45.61 & 59.64            \\
vessel                    & 0.397 & -        & 0.530           & 0.502 & \textbf{0.552}   & 0.212 & \textbf{0.151 } & 0.218            & 0.208 & 0.173           & \textbf{49.87}  & 42.37            & 36.04 & 45.88            \\ 
\midrule
mean                      & 0.480 & -        & \textbf{0.571}  & 0.499 & 0.567            & 0.216 & \textbf{0.175 } & 0.215            & 0.349 & 0.245           & 48.57           & \textbf{51.75 }  & 34.86 & 47.36            \\
\bottomrule
\multicolumn{15}{c}{\textbf{RGB-to-3D} }
\end{tabular}

} %< resizebox
\end{center}
\drawmyfilename{}
\vspace{\baselineskip}
\caption{
% 
\textbf{Reconstruction performance on ShapeNet/Multi} --
% 
We evaluate our method against \PtoM{}, \AtlasNet{}, \OccNet{} and 
\SIF{}. We provide in input either (left) a collection of depth maps or (right) a single color image.
For \AtlasNet{}, note that IoU cannot be measured as the meshes are not watertight.
We omit \VP{}, as it only produces a very rough shape decomposition.
% 
\TODO{THIS VERSION INCLUDES THE POINT CLOUD + POINTNET VERSION OF OCCNET -- SIMPLER PROBLEM, BUT COMPARES IT TO THE DEPTH VERSION OF OTHER METHODS}
% 
% \BD{The highlight in the RGB-to-3D table seems weird.}
% \AT{the vertical bars in the right table are a bit weird?}
% \BD{I think the quantitative results are more important for multi-class. For single class experiments, our focus is structure or correspondence. So I think we may consider find another quantitative measure rather than adding another 2 lines here.}
% 
}
\label{tbl:shapenet}
\end{table*}
